Graded and Geometric Parabolic Induction for Category $\mathcal{O}$

We prove that the parabolic induction functor on BGG-category $\mathcal{O}$ associated to a complex reductive Lie algebra is gradable, that is, lifts to graded category $\mathcal{O}$ as constructed by Beilinson-Ginzburg-Soergel. Graded category $\mathcal{O}$ is equivalent to a category of stratified mixed Tate motives on a corresponding flag variety as recently defined by Soergel-Wendt. The graded version of parabolic induction is induced by a geometric parabolic induction functor we construct on the level of stratified mixed Tate motives. We also describe the effect of parabolic induction on the level of Soergel modules.

==> Inhalt/introduction.tex <==
\section{Introduction}

==> Inhalt/soergelmodules <==
\chapter{Soergel modules and main results}
